Federated Learning with Compression: Unified Analysis and Sharp Guarantees

In federated learning, communication cost is often a critical bottleneck to scale up distributed optimization algorithms to collaboratively learn a model from millions of devices with potentially unreliable or limited communication and heterogeneous data distributions. Two notable trends to deal with the communication overhead of federated algorithms are gradient compression and local computation with periodic communication. Despite many attempts, characterizing the relationship between these two approaches has proven elusive. We address this by proposing a set of algorithms with periodical compressed (quantized or sparsified) communication and analyze their convergence properties in both homogeneous and heterogeneous local data distribution settings. For the homogeneous setting, our analysis improves existing bounds by providing tighter convergence rates for both strongly convex and non-convex objective functions. To mitigate data heterogeneity, we introduce a local gradient tracking scheme and obtain sharp convergence rates that match the best-known communication complexities without compression for convex, strongly convex, and nonconvex settings. We complement our theoretical results and demonstrate the effectiveness of our proposed methods by several experiments on real-world datasets.

==> commands.tex <==
\usepackage{epsf}
%\usepackage{fancyheadings}
\usepackage{graphics}
%\usepackage{graphicx}

%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage{psfrag}

\usepackage{color}

\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{fdsymbol}
%\usepackage[linesnumbered, ruled, vlined]{algorithm2e}
%\usepackage{ntheorem}

%\usepackage[backend=bibtex,firstinits=true]{biblatex}

%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS HERE

%%%%%%%
%\theoremstyle{plain}

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper

%\theoremprework{\begin{minipage}{\textwidth}}
%\theorempostwork{\end{minipage}}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
%\newlength{\widebarargwidth}
%\newlength{\widebarargheight}
%\newlength{\widebarargdepth}
%\DeclareRobustCommand{\widebar}[1]{%
%  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
%  \settoheight{\widebarargheight}{\ensuremath{#1}}%
%  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
%  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
%    \hspace{0.3\widebarargdepth}%
%    \addtolength{\widebarargheight}{0.3ex}%
%    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
%  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
%\makeatletter
%\long\def\@makecaption#1#2{
%        \vskip 0.8ex
%        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
%        \parindent 1.5em  %% How can we use the global value of this???
%        \dimen0=\hsize
%        \advance\dimen0 by -3em
%        \ifdim \wd\@tempboxa >\dimen0
%                \hbox to \hsize{
%                        \parindent 0em
%                        \hfil 
%                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
%                                {\bf #1.} #2
%                                %%\unhbox\@tempboxa
%                                } 
%                        \hfil}
%        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
%        \fi
%        }
%\makeatother



%% COMMENTING commands

\long\def\comment#1{}

\newcommand{\bm}[1]{\boldsymbol{#1}}
\newcommand{\bit}[1]{\boldsymbol{#1}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mjwcomment}[1]{{\bf{{\red{{MJW --- #1}}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\mycomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\vidyacomment}[1]{{\bf{{\green{{VM --- #1}}}}}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\cmcomment}[1]{{\bf{{\cyan{{CM --- #1}}}}}}

% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

\newcommand{\defn}{:\,=}

%Hamming metric
\newcommand{\dH}{\mathsf{d}_{\mathsf{H}} }

\newcommand{\id}{\mathsf{id}}

\newcommand{\KT}{\mathsf{KT}}

\newcommand{\dimone}{n_1}
\newcommand{\dimtwo}{n_2}
\newcommand{\maxdimonetwo}{\left(\dimone \lor \dimtwo \right)}

\newcommand{\Aone}{{\bf C1} }
\newcommand{\Atwo}{{\bf C2} }

\newcommand{\csst}{\mathbb{C}_{\mathsf{SST}}}
\newcommand{\cdiff}{\mathbb{C}_{\mathsf{DIFF}}}
\newcommand{\Cpara}{\mathbb{C}_{\mathsf{PARA}}}
\newcommand{\Cbiso}{\mathbb{C}_{\mathsf{BISO}}}
\newcommand{\Cns}{\mathbb{C}_{\mathsf{NS}}}
\newcommand{\Cnspi}{M_{\mathsf{NS}, \pi}}
\newcommand{\Mns}{M_{\mathsf{NS}}}
\newcommand{\Cnspihat}{M_{\mathsf{NS}, \pihat}}

\newcommand{\sk}{S_k}
\newcommand{\bl}{\mathsf{bl}}

\newcommand{\bltilde}{\widetilde{\mathsf{bl}}}
\newcommand{\Bl}{\mathsf{B}}
\newcommand{\Rw}{\mathsf{R}}

\newcommand{\tauhat}{\widehat{\tau}}
\newcommand{\Chatt}{\widehat{C}_t}

\newcommand{\rhat}{\widehat{\mathsf{r}}}
\newcommand{\rspace}{\mathsf{r}}

\newcommand{\elts}{\mathsf{s}}
\newcommand{\Ntilde}{\widetilde{N}}

\newcommand{\lambdahat}{\widehat{\lambda}}

\newcommand{\Cmodel}{\mathbb{C}}

\newcommand{\pobs}{p_{\mathsf{obs}}}

\newcommand{\sgn}{\mathsf{sgn}}

\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{fro}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}


% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% Kullback-Leibler
\newcommand{\kull}[2]{\ensuremath{D(#1\; \| \; #2)}}

% Probability
\newcommand{\E}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

% Observations, dimension etc.
\newcommand{\numobs}{\ensuremath{n}}
\newcommand{\usedim}{\ensuremath{d}}

\newcommand{\Comp}{\ensuremath{C}}

\newcommand{\Mrisk}{\ensuremath{\mathcal{M}}}
\newcommand{\Erisk}{\ensuremath{\mathcal{E}}}
\newcommand{\Arisk}{\ensuremath{\mathcal{A}}}

\newcommand{\diam}{\ensuremath{\mathsf{diam}}}
%Numbering
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}

\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\child}{child}
\DeclareMathOperator{\parent}{parent}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{{\sf rank}}
\DeclareMathOperator{\card}{{\sf card}}
\DeclareMathOperator{\range}{{\sf range}}
\DeclareMathOperator{\toeplitz}{toeplitz}


% 
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}
\newcommand{\Ospace}{\ensuremath{\mathcal{O}}}

\newcommand{\Bupper}{\ensuremath{\overline{B}}}
\newcommand{\Blower}{\ensuremath{\underline{B}}}
% Basic statistics notation
% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimate one
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}

\newcommand{\xhat}{\ensuremath{\widehat{x}}}
\newcommand{\Deltahat}{\ensuremath{\widehat{\Delta}}}

\newcommand{\Deltatilde}{\ensuremath{\widetilde{\Delta}}}
\newcommand{\udiff}{\ensuremath{\mathbb{U}^{{\sf diff}}_m(A)}}
\newcommand{\Xhat}{\ensuremath{\widehat{X}}}
\newcommand{\Yhat}{\ensuremath{\widehat{Y}}}
\newcommand{\Ytilde}{\ensuremath{\widetilde{Y}}}
\newcommand{\Mhat}{\ensuremath{\widehat{M}}}
\newcommand{\Mstar}{\ensuremath{M^*}}
\newcommand{\Mtilde}{\ensuremath{\widetilde{M}}}
\newcommand{\bhat}{\ensuremath{\widehat{b}}}
\newcommand{\Mhatasp}{\ensuremath{\widehat{M}}_{\mathsf{ASP}}}
\newcommand{\ASP}{\ensuremath{\mathsf{ASP}}}

\newcommand{\CRL}{\ensuremath{\mathsf{CRL}}}

\newcommand{\Mhattds}{\ensuremath{\widehat{M}}_{{\sf TDS}}}

\newcommand{\Mhatod}{\ensuremath{\widehat{M}}_{{\sf 1D}}}
\newcommand{\Mhatls}{\ensuremath{\widehat{M}}_{{\sf LS}}}
\newcommand{\Mhatpermr}{\ensuremath{\widehat{M}}_{{\sf permr}}}

\newcommand{\BAP}{\ensuremath{\mathsf{BAP}}}
\newcommand{\agg}{\ensuremath{\mathsf{Agg}}}
\newcommand{\Mhatbap}{\ensuremath{\widehat{M}}_{\mathsf{BAP}}}

\newcommand{\Btilde}{\ensuremath{\widetilde{B}}}

\newcommand{\xhatml}{\ensuremath{\widehat{x}_{{\sf ML}}}}
\newcommand{\Xhatml}{\ensuremath{\widehat{X}_{{\sf ML}}}}
% Estimate two
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

\newcommand{\gt}{\ensuremath{\widetilde{g}}}

\newcommand{\yvec}{\ensuremath{y}}
\newcommand{\Xmat}{\ensuremath{X}}

\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}


%Problem-specific notation
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
\newcommand{\real}{\ensuremath{\mathbb{R}}}

\newcommand{\Pihat}{\ensuremath{\widehat{\Pi}}}
\newcommand{\pihat}{\ensuremath{\widehat{\pi}}}
\newcommand{\pihatborda}{\ensuremath{\widehat{\pi}_{\sf bor}}}
\newcommand{\pihatpre}{\ensuremath{\widehat{\pi}_{\sf pre}}}
%\newcommand{\pihatref}{\ensuremath{\widehat{\pi}_{\sf ref}}}
\newcommand{\pihattds}{\ensuremath{\widehat{\pi}_{\sf tds}}}
\newcommand{\pihatoned}{\ensuremath{\widehat{\pi}_{{\sf 1D}}}}
\newcommand{\pihatftds}{\ensuremath{\widehat{\pi}_{{\sf tds}}}}
\newcommand{\sigmahat}{\ensuremath{\widehat{\sigma}}}
\newcommand{\Sigmahat}{\ensuremath{\widehat{\Sigma}}}
\newcommand{\sigmahatborda}{\ensuremath{\widehat{\sigma}_{\sf bor}}}
%\newcommand{\sigmahatref}{\ensuremath{\widehat{\sigma}_{\sf ref}}}
\newcommand{\sigmahattds}{\ensuremath{\widehat{\sigma}_{\sf tds}}}
\newcommand{\sigmahatftds}{\ensuremath{\widehat{\sigma}_{\sf tds}}}
\newcommand{\sigmahatpre}{\ensuremath{\widehat{\sigma}_{\sf pre}}}

\newcommand{\pihatasp}{\ensuremath{\widehat{\pi}_{\mathsf{ASP}}}}
\newcommand{\Pihatml}{\ensuremath{\widehat{\Pi}_{{\sf ML}}}}
\newcommand{\Pitil}{\ensuremath{\widetilde{\Pi}}}

\newcommand{\Projpi}{\ensuremath{P_{\Pi}}}
\newcommand{\Projorthpi}{\ensuremath{P_{\Pi}^{\perp}}}
\newcommand{\Projorthpistar}{\ensuremath{P_{\Pi^*}^{\perp}}}

\newcommand{\hballpi}{\ensuremath{\mathbb{B}^{\sf H}_\Pi}}
\newcommand{\hballpistar}{\ensuremath{\mathbb{B}_{\sf H}}}
%\newcommand{\hballpistar}{\ensuremath{\mathcal{P}_n}}
\newcommand{\SNR}{\ensuremath{\frac{\|x^*\|_2^2}{\sigma^2}}}
\newcommand{\col}{\ensuremath{{\sf col}}}
\newcommand{\row}{\ensuremath{{\sf row}}}
\newcommand{\Pn}{\ensuremath{\mathcal{P}_n}}

\newcommand{\EE}{\ensuremath{\mathbb{E}}}
%changed to probability of error
\newcommand{\Rpihat}{\ensuremath{\Pr\{ \Pihat \neq \Pi^* \} }}

\newcommand{\Rpihatml}{\ensuremath{\Pr\{ \Pihatml \neq \Pi^* \}}}
\newcommand{\BigO}{\ensuremath{\mathcal{O}}}


\newcommand{\numitems}{\ensuremath{n}}

% commands that CM changed/introduced
\newcommand{\symgp}{\mathfrak{S}}
\newcommand{\vars}{\zeta}
\newcommand{\maxvarone}{(\vars^2 \lor 1)}
\newcommand{\varplusone}{(\vars + 1)}
\newcommand{\allones}{\mathbf{e}}
\newcommand{\bfone}{\mathbf{1}}
\DeclareMathOperator{\trace}{\mathsf{tr}}
\DeclareMathOperator{\Poi}{\mathsf{Poi}}
\DeclareMathOperator{\var}{\mathsf{var}}
\DeclarePairedDelimiter\tv{\mathsf{tv}(}{)}

%\newcommand{\Cperm}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{r},\mathsf{c}}}
\newcommand{\Cperm}{\mathbb{C}_{\mathsf{Perm}}}
%\newcommand{\Cpermr}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{r}}}
%\newcommand{\Cpermc}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{c}}}
\newcommand{\Cskew}{\mathbb{C}_{\mathsf{skew}}}

\newcommand{\tds}{{\sf TDS}}

\newcommand{\Ypoi}{Y_{\sf Poi}}
%\newcommand{\Ysortcol}{Y_{\sf sortcol}}
%\newcommand{\Ysortrow}{Y_{\sf sortrow}}

\newcommand{\BL}{\mathsf{BL}}

\newcommand{\Mps}{M_{\pi, \sigma}}
\newcommand{\Dps}{\Delta_{\pi, \sigma}}
\newcommand{\Cdiffps}{\cdiff(\pi, \sigma)}
\newcommand{\Zps}{Z_{\pi, \sigma}}
\newcommand{\Ztil}{\Zps}
\newcommand{\At}{\mathcal{A}_t}
\newcommand{\Wtil}{\widetilde{W}}
\newcommand{\cE}{\mathcal{E}}

\newcommand{\bllarge}{\mathsf{BL}^{\mathbb{L}}}
\newcommand{\blsmall}{\mathsf{BL}^{\mathbb{S}}}
%\newcommand{\blunion}{\cup \mathsf{bl}}
%\newcommand{\bllargeunion}{\cup \bllarge}
%\newcommand{\blsmallunion}{\cup \blsmall}
\newcommand{\blone}{\BL^{(1)}}
\newcommand{\bltwo}{\BL^{(2)}}
%\newcommand{\blthree}{\BL^{(3)}}
\newcommand{\blt}{\BL^{(t)}}
%\newcommand{\bltp}{\BL^{(t')}}

\newcommand{\blocksize}{\dimtwo \sqrt{\frac{\dimone}{N} \log (\dimone \dimtwo) }}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

